In-depth Analysis of Densest Subgraph Discovery in a Unified Framework

As a fundamental topic in graph mining, Densest Subgraph Discovery (DSD) has found a wide spectrum of real applications. Several DSD algorithms, including exact and approximation algorithms, have been proposed in the literature. However, these algorithms have not been systematically and comprehensively compared under the same experimental settings. In this paper, we first propose a unified framework to incorporate all DSD algorithms from a high-level perspective. We then extensively compare representative DSD algorithms over a range of graphs -- from small to billion-scale -- and examine the effectiveness of all methods. Moreover, we suggest new variants of the DSD algorithms by combining the existing techniques, which are up to 10 X faster than the state-of-the-art algorithm with the same accuracy guarantee. Finally, based on the findings, we offer promising research opportunities. We believe that a deeper understanding of the behavior of existing algorithms can provide new valuable insights for future research. The codes are released at https://anonymous.4open.science/r/DensestSubgraph-245A

==> sections/4_Compare/Verify.tex <==
\subsection{Verification}
\label{sec:verify}
In this section, we explain how to check if a candidate subgraph is the exact solution or if it meets the approximation ratio requirement.
%
All exact algorithms need to verify their candidate subgraphs, and the approximation algorithms except the peeling-based need to do this step.

\textbf{FlowExact and CoreExact.} {\tt FlowExact} checks if the difference between $\overline{\rho}$ and $\underline{\rho}$ is less than $ \frac{1}{n \cdot (n - 1)}$, as the density difference between any two graphs must be larger than $\frac{1}{n \cdot (n - 1)}$.
%
When the condition is satisfied, the exact solution has been found.
    
{\tt CoreExact} utilizes  less stringent  stop conditions for verifying results:
$\frac{1}{|V_C| \cdot (|V_C| - 1)}$,
where $V_C$ is the largest connected component in the graph.



\textbf{CP-based Exact Algorithms.} 
  

==> sections/5_Directed/Optimizations.tex <==
\subsection{Optimization Methods}
\label{sec:dds_optimize}




==> sections/5_Directed/definition.tex <==
% \subsection{Preliminaries}


\begin{definition}[ {$[ x, y ]$}-core \cite{ma2020efficient}]
\label{def:x-y-core}
Given a directed graph $D$=($V$, $E$), the {\bf $[x$, $y]$-core} is the largest ($S$, $T$)-induced subgraph $D[S,T]$, which satisfies:
\begin{enumerate}
	\item $\forall u \in S, d^{+}_{D[S,T]}(u) \geq x$ and $\forall v \in T, d^{- }_{D[S,T]}(v) \geq y$;
	\item $\nexists D[S', T']\neq D[S,T]$, such that $D[S,T]$ is a subgraph of $D[S',T']$, i.e., $S \subseteq S'$, $T \subseteq T'$, and $D[S',T']$ satisfies (1);
\end{enumerate}
where $d^{+}_{D[S,T]}(u)$ is the out-degree of $u$ in $D[S,T]$ and $d^{- }_{D[S,T]}(v)$ is the in-degree of $v$ in $D[S,T]$. $[x^{*}, y^{*}]$-core denotes the $[x, y]$-core with the largest $x \cdot y$ among all $[x, y]$-cores.
\end{definition}

\begin{definition} [$c$-biased density\cite{ma2022convex}]
    Given a directed graph $D$=$(V,E)$, a fixed $c$ and two vertex sets $S$ and $T$, the $c$-biased density of an ($S$, $T$)-induced subgraph is proportional to its edge-density, and is defined as 
$\rho_c(S, T)= \frac{2\sqrt{c}\sqrt{c'}}{c+c'}\rho (S, T) = \frac{2\sqrt{c}\sqrt{c'}}{c+c'}\frac{{|E(S, T)|}}{{\sqrt{|S||T|}}}
$, where $c'=\frac{|S|}{|T|}$. Note when $c'=c$, $\rho_c(S, T)=\rho(S,T)$.
\end{definition}

\begin{definition} [$c$-biased directed densest subgraph (DDS)~\cite{ma2022convex}]
    Given a directed graph $D$ and a fixed $c$, the subgraph, whose corresponding $c$-biased density is the highest among all possible ones, is called the $c$-biased DDS.
\end{definition}
% For ease of exposition, we will use $G[S^{*}, T^{*}]$ to denote the densest subgraphs in the directed graphs.



Besides, Ma.et al \cite{ma2022convex}
present the convergence of employing Frank-Wolfe algorithm to solve \Cref{equ:ma-dual-lp}, which is given by the following theorem:
\begin{theorem}[\cite{ma2022convex}]
Given a directed graph $D$ and $c$, suppose \(d_{\text{max}}^\text{+}\) (resp. \(d_{\text{max}}^\text{-}\)) is the maximum out-degree (resp. in-degree) of \(D\). For $t > 16\frac{\kappa m}{\varepsilon^2}$, we have $\| \max_{u \in V} \{|\mathbf{w}_{\alpha}(u)|,  |\mathbf{w}_{\beta}(u)|\}\|_\infty - \rho_D^* \le \varepsilon$, where $\kappa = \sum_{c\in C}(\sqrt{c} + \frac{1}{\sqrt{c}})\max\{\sqrt{c} d_{\text{max}}^{+}, \frac{1}{\sqrt{c}} d_{\text{max}}^-\}$, and $C$ = $\{\frac{a}{b} \mid 1\le a, b\le n\}$.
\end{theorem}

% where $\mathbf{w}$ is the vertex weight vector:
% \begin{equation*}
%     \mathbf{w} =  \begin{bmatrix} \mathbf{w}_{\alpha}(v_1) , \mathbf{w}_{\alpha}(v_2), \cdots, \mathbf{w}_{\alpha}(v_n),  \mathbf{w}_{\beta}(v_1), \mathbf{w}_{\beta}(v_2), \cdots, \mathbf{w}_{\beta}(v_n) \end{bmatrix} 
% \end{equation*}



==> sections/6_Experiment/application.tex <==

\subsection{Case studies}
\label{sec:exp:apply}

In this section, we present two case studies on real-world HINs.

{\it (1) Community discovery.} We consider the DBLP co-authorship network and use {\tt POMA} to find groups of researchers and papers by using a motif, i.e.,  ``Author-Paper-Author'', which is also a meta-path \cite{DBLP:journals/pvldb/SunHYYW11}, describing the co-authorship between two authors.
%
Intuitively, we wish to find cohesive heterogeneous communities, each of which includes both authors and papers that are intensively linked together.
%
Figure \ref{fig:case-dblp}(c) depicts a maximal M-clique based on the motif, showing that the four researchers ``Jiawei Han'', ``Jian Pei'', ``Yizhou Sun'', and ``Philip S. Yu'' have very close collaboration on  four papers in Figure \ref{fig:case-dblp}(b).

\begin{figure}[h]
    \centering
    \includegraphics[scale=0.372]{figures/case_study_dblp.pdf}
    \caption{A case study on DBLP co-authorship network.}
    \label{fig:case-dblp}
\end{figure}

{\it (2) Product recommendation.} We use the Instacart e-commerce network which includes various products.
%
We consider a 4-vertex motif with three types of items (i.e., ``beverages'', ``daily egg'',  and ``snack''), as shown in Figure \ref{fig:instacart}(a).
%
The intuition of this motif is to find out those beverages and daily egg products that are frequently bought together with snacks for better product promotion.
%
Figure \ref{fig:instacart}(b) shows a maximal M-clique found by {\tt POMA}, which is highly connected and reflects the related items interesting to customers.
%
Thus, the maximal M-clique can be used in product promotion (e.g., a bundle containing two snacks, one beverage, and one daily egg extracted from this maximal M-clique might be sold at a discounted price).

\begin{figure}[h]
    \centering
    \includegraphics[scale=0.39]{figures/case_study_instacart.pdf}
    \caption{A case study on Instacart e-commerce network.}
    \label{fig:instacart}
\end{figure}

In addition, we would like to bring to the readers' attention that a recent demo system \cite{li2020mc} has shown the various applications of maximal M-cliques in biological network analysis.
%
As shown in \cite{li2020mc}, the maximal M-clique can be used to disclose new side effects of a drug and potential drugs for healing diseases on a large biological network, facilitate the analysis and visualization of a biological network, support disease subtyping, drug mechanism investigation, and drug repurposing.
%
An online video demonstrating how the maximal M-clique works for the above applications is available at \underline{\url{https://www.dropbox.com/s/vkalumc28wqp8yl/demo.mov}}.
